Sublinear Estimation of Weighted Matchings in Dynamic Data Streams

This paper presents an algorithm for estimating the weight of a maximum weighted matching by augmenting any estimation routine for the size of an unweighted matching. The algorithm is implementable in any streaming model including dynamic graph streams. We also give the first constant estimation for the maximum matching size in a dynamic graph stream for planar graphs (or any graph with bounded arboricity) using $\tilde{O}(n^{4/5})$ space which also extends to weighted matching. Using previous results by Kapralov, Khanna, and Sudan (2014) we obtain a $\mathrm{polylog}(n)$ approximation for general graphs using $\mathrm{polylog}(n)$ space in random order streams, respectively. In addition, we give a space lower bound of $\Omega(n^{1-\varepsilon})$ for any randomized algorithm estimating the size of a maximum matching up to a $1+O(\varepsilon)$ factor for adversarial streams.

==> unweighted_matching.tex <==
%\begin{algorithm}[h]
%\label{alg1}
%\caption{\bf{Unweighted Matching Approximation}}
%%\LinesNumbered
%\SetKwData{I}{i}
%\SetKwInOut{Input}{input}
%\Input{$G=(V,E)$, $\varepsilon > 0$}
%$F\leftarrow V$\;
%$estimate_1 \leftarrow 0$\;
%\lnlset{InResR}{Phase 1}%
%\For{$i=1 ${\bf{ to }$r$}}{
%$E'\leftarrow \emptyset$\;
%\For{$v\in F$}{
%\For{$j=1 ${\bf{ to }$\sqrt{n} \cdot \log^2 n$}}{
%Sample random neighbor $u$ from $v$\;
%\If{$u\in F$}{
%$E' \leftarrow E'\cup \{(v,u)\}$\;
%break\;
%}
%}
%}
%$M\leftarrow \text{maximal matching }(F,E')$\;
%$estimate_1 \leftarrow estimate_1 + |M|$\;
%remove matched nodes from $F$\;
%}
%\lnlset{InResR}{Phase 2}%
%$M' \leftarrow \emptyset$\;
%$count \leftarrow 0$\;
%\For{$j=1 ${\bf{ to }$s$}}{
%Sample a random edge $e = (u,v)$ from $E(F)$\;
%\If{$u$ and $v$ are free w.r.t. $M'$ or $e \in M'$}{
%$count \leftarrow count + 1$\;
%$M' \leftarrow M' \cup e$\;
%}
%}
%%$M\leftarrow \text{maximal matching }(F,E')$\;
%$estimate_2 \leftarrow count \cdot \frac{|E(F)|}{s}$\;
%$estimate \leftarrow estimate_1 + estimate_2$\;
%\Return $estimate$\;
%\end{algorithm}
%
%\section{Unweighted Matching}
%We first describe an offline estimation of the maximum matching and then show how to implement it in the dynamic streaming setting.
%The algorithm proceeds in two phases. In the first phase we emulate a parallel maximal matching algorithm by Israeli and Itai~\cite{IsI86}. We now briefly sketch their algorithm to make this paper self-contained.
%Every unmatched node chooses an adjacent unmatched node uniformly at random. Among all thus chosen edges a maximal matching is computed and added to the global matching. All matched nodes and incident edges are deleted from the graph and the procedure is repeated until no edges remain. The algorithm terminates after an expected number of $O(\log n)$ rounds and with high probability after $O(\log^2 n)$ rounds.
%Once our first phase is completed, we have either computed a sufficiently good approximation to a maximal matching, or the graph will be sufficiently sparse to execute the estimation routine of the second phase, which consists of sampling a sufficient number of randomly chosen edges from all unmatched nodes, computing a maximal matching and rescaling the result.
%
%
%
%\begin{proof}[Proof of Theorem~\ref{thm:unweightedstream}]
%We first show that after $O(\sqrt{n}\cdot \text{log}^4 n)$ iterations all unmatched nodes $v\in F$ have $\text{deg}_F(v)\leq \frac{1}{\sqrt{n}} \cdot \text{deg}(v)$. 
%If $\text{deg}_F(v)\geq \frac{1}{\sqrt{n}}\cdot \text{deg}(v)$, we will sample a node $u\in F$ in line 7 with at least probability $\frac{1}{\sqrt{n}}$. 
%Hence after $\sqrt{n}\cdot \log n^2$ iterations, we do not sample a node from $F$ with probability at most $(1-\frac{1}{\sqrt{n}})^{\sqrt{n}\cdot \log n^2} \leq e^{-\log n^2} =\frac{1}{n^2}$. 
%Applying a union bound over $n$ nodes gives us the same statement that we sample an unmatched neighbor for all free nodes $v$ with  $\text{deg}_F(v)\geq \frac{1}{\sqrt{n}}\cdot \text{deg}(v)$ with high probability. Now we may reapply the analysis of Israeli and Itai~\cite{IsI86}, leading to the fact that after each iteration the number of edges incident to free nodes $v$ with $\text{deg}_F(v)\geq \frac{1}{\sqrt{n}}\cdot \text{deg}(v)$ is halved in expectation and after $r \in O(\log^2 n)$ many iterations all free nodes $v$ have $\text{deg}_F(v)\leq \frac{1}{\sqrt{n}} \cdot \text{deg}(v)$ with high probability. 
%%Hence, we require at most $O(n^{\epsilon}\log^4 n)$ iterations.
%
%For the second estimator, we require the following  lemma which is a simple application of Chebyshev's inequality.
%
%\begin{lemma}
%\label{lem:trivialest}
%Let $G(V,E)$ be an unweighted undirected graph and let $M$ be any maximal matching on $G$. Let $E'$ be a set of $s$ uniformly sampled subset of $E$. For each edge $e\in E'$ denote by $X_e$ the binary random variable indicating if $e$ is a matching edge of $M$, that is 
%$ X_e = 1$ iff $ e\in M$. Then we have
%\[\mathbb{P}\left[ \left| \sum_{e\in E'} X_e\cdot \frac{|E|}{s}-|M| \right| < t\right] > \frac{1}{2}\]
%if $s\geq \frac{2 \cdot |E|\cdot |M|}{t^2}$.
%\end{lemma}
%\begin{proof}
%%Fix a maximal matching $M$.
%%For each edge $e\in E'$ denote by $X_e$ the binary random variable indicating if $e$ is a matching edge of $M$, that is $X_e = \begin{cases} 1 &\text{if } e\in M\\
%%0 &\text{otherwise}\end{cases}$. Then for the first and second moments of the estimator we have
%%\begin{equation}
%%\label{eq:firstmom}
%%\mathbb{E}\left[\sum_{e\in E'} X_e\cdot \frac{|E|}{s}\right] = \frac{|E|}{s}\cdot\sum_{e\in E'}\mathbb{P}[X_e] = \frac{|E|}{s}\cdot s\cdot \frac{|M|}{|E|} = |M|
%%\end{equation}
%%and
%%\begin{eqnarray}
%%\nonumber
%%\mathbb{E}\left[\left(\sum_{e\in E'} X_e\cdot \frac{|E|}{s}\right)^2\right] &=& \frac{|E|^2}{s^2}\cdot \mathbb{E}\left[\sum_{e\in E'} X_e^2+\sum_{e\neq e'\in E'}X_e\cdot X_{e'}\right] \\
%%\nonumber
%%&=& \frac{|E|^2}{s^2}\cdot\left(s\cdot \mathbb{P}[X_e^2] + {s\choose 2}\cdot\mathbb{P}[X_e]\cdot\mathbb{P}[X_{e'}]\right)\\
%%\nonumber
%%&= & \frac{|E|^2}{s^2}\cdot \left(s\cdot \frac{|M|}{|E|} + \frac{s\cdot(s+1)}{2}\cdot\frac{|M|^2}{|E|^2}\right) \\
%%\label{eq:secondmom}
%%&\leq & \frac{|E|\cdot |M|}{s} + |M|^2
%%\end{eqnarray}
%For every $e \in E'$ it is
%$$\text{Var}\left[ X_e \right] = \dfrac{\vert M \vert}{\vert E \vert} - \dfrac{\vert M \vert^2}{\vert E \vert^2} \leq \dfrac{\vert M \vert}{\vert E \vert}. $$
%We then have
%\begin{eqnarray}
%\label{eq:chebyshev}
%\mathbb{P}\left[ \left| |M'|\cdot \frac{|E|}{s}-|M| \right| \geq t\right] &\leq & \frac{\text{Var}\left[\sum_{e\in E'} X_e\cdot \frac{|E|}{s}\right]}{t^2}\\
%\label{eq:independence}
%& = &  \frac{\frac{|E|^2}{s^2} \sum_{e\in E'} \text{Var}\left[ X_e \right]}{t^2}\\
%\nonumber
%& \leq & \frac{|E|\cdot |M|}{s \cdot t^2}
%%\nonumber
%%&=&  \frac{|E|\cdot |M| }{s\cdot t^2},
%\end{eqnarray}
%where (\ref{eq:chebyshev}) follows from Chebyshev and (\ref{eq:independence}) follows from the independence of the $X_e$ variables.
%%standard variance decomposition for any random variable ($\text{Var}(X)=\mathbb{E}[X^2]-\mathbb{E}[X]^2$) and Equations~\ref{eq:firstmom} and~\ref{eq:secondmom}. 
%\end{proof}
%
%We now show how to estimate the size of the maximum matching of the subgraph remaining after phase 1. 
%A sufficiently good estimation then yields a $(1\pm\epsilon)$ approximation to a maximal matching of $G$.
%Let $G'(F,E(F))$ and $u=\underset{v\in F}{\text{argmax }}\text{deg}(v)$. 
%Then the size of the matching computed in phase 1 can be lower bounded by $\frac{1-\frac{1}{\sqrt{n}}}{2}\cdot \text{deg}(u)$. 
%At the same time, the number of edges contained in $E(F)$ can be upper bounded by $F\cdot \frac{1}{\sqrt{n}}\cdot \text{deg}(u)\leq \sqrt{n}\cdot \text{deg} (u)$. 
%Thus, if a maximal matching $M$ of $G'$ is of size at least $\frac{1-\frac{1}{\sqrt{n}}}{2}\cdot \text{deg}(u)$, we obtain an $(1\pm \epsilon)$ approximation to the size of a maximal matching with constant probability via Lemma~\ref{lem:trivialest} by setting $t=\epsilon\cdot |M|$ and hence 
%\[s\geq 4\cdot \frac{\sqrt{n}\cdot \text{deg}(u)}{(1-\frac{1}{\sqrt{n}})\cdot \text{deg}(u)}\cdot \epsilon^{-2} \geq 2 \cdot \frac{|E(F)|\cdot |M|}{\epsilon^{2}\cdot|M|^2} =2\cdot\frac{|E(F)|\cdot |M|}{t^2}.\]
%If on the other hand the maximum matching $M$ is of size less than $\frac{1-\frac{1}{\sqrt{n}}}{2}\cdot \text{deg}(u)$ and in particular of size less than the matching already computed on $V\setminus F$, it is sufficient to estimate $|M|$ up to an $t=\epsilon\cdot \frac{1-\frac{1}{\sqrt{n}}}{2}\cdot \text{deg}(u)$ additive error. Again, setting 
%\[s \geq 4\cdot \frac{\sqrt{n}\cdot \text{deg}(u)}{(1-\frac{1}{\sqrt{n}})\cdot \text{deg}(u)}\cdot \epsilon^{-2} \geq 2 \cdot \frac{|E(F)|\cdot |M|}{\epsilon^2\cdot \left(\frac{1-\frac{1}{\sqrt{n}}}{2}\cdot \text{deg}(u)\right)^2} = 2 \cdot\frac{ |E(F)|\cdot |M|}{t^2}\]
%gives us a $(1\pm\epsilon)$ approximation to a maximal matching of $G'$ with constant probability. 
%
%Amplifying the second estimator in the standard way and adding both estimations gives us a $(1\pm\epsilon)$-approximation to the cardinality of a maximal matching in $G$ with high probability using $O\left(n^{3/2}\log^3 n + \sqrt{n}\cdot \epsilon^{-2}\cdot \log n \right)$ many sampled edges. Let $OPT$ be the size of a maximum matching in $G$. Since the size of a maximal matching is at least $1/2\cdot OPT$ and at most $OPT$, we obtain an estimator which is at least $(1/2-\epsilon/2) \cdot OPT$ and at most $(1+\epsilon)\cdot OPT$.
%
%\subsection{Streaming Implementation}
%%First, note that there is a trade-off between the number of edges sampled in phase 1 and phase 2. This observation is quite important to understand why our streaming implementation needs roughly $O(n^{1+\varepsilon} + n^{2-\varepsilon})$ space. For every sampled edge in phase 1 we need an $\ell_0$ sampler resulting in $\tilde{O}(n^{1+\varepsilon})$ space. If we were able to maintain a sketch such that we can sample from $E(F)$ and $F$ is updated over time, we could directly apply the standard greedy algorithm to compute a maximal matching. So the difficulty in phase 2 is to sample enough edges from $E(F)$. 
%
%\subparagraph*{Phase 1} The first phase of Algorithm~\ref{alg1} is readily adapted to the streaming setting by maintaining a $\left(0,\frac{1}{n^2}\right)$ $\ell_0$ sampler for every sampled neighbor of every node $v\in V$, leading to an overall space requirement of $O\left(n^{3/2}\log^7 n\right)$ for this phase.
%\subparagraph{Phase 2} The adaptation of the sampling procedure in the second phase is more involved, as our sample must be chosen uniformly from among all edges only incident with unmatched nodes. Maintaining a sketch for this set of edges such that we can directly sample from it seems quite difficult since we do not know the unmatched nodes in advance. Instead we obliviously sample $\tilde{O}\left(n^{3/2}\right)$ edges $S$ from the whole edge set $E$ and show that we sample enough edges from $E(F)$ with a little more involved case study than in the last section.
%
%Let $M_1$ be the maximal matching in phase $1$, \ie $estimate_1 = \vert M_1 \vert$. Fix any maximal matching $M_2$ in the remaining graph of phase 2, \ie $G(V,E(F))$. We condition all following statements on the high probability event that the sample $S$ contains at least $2 \cdot n^{3/2} \cdot \frac{\vert E(F) \vert}{\vert E \vert}$ edges from $E(F)$ (amplifying the probability with additional samples).
%\begin{enumerate}
%\item $\vert M_2 \vert \geq \dfrac{\sqrt{n}}{\varepsilon^2}$: We set $t = \varepsilon \vert M_2 \vert$. Then we have 
%$$ s \geq 2 \cdot n^{1.5} \cdot \frac{\vert E(F) \vert}{\vert E \vert} \geq 2 \cdot \dfrac{\vert E(F) \vert}{\sqrt{n}} \geq  2 \cdot \dfrac{\vert E(F) \vert}{ \varepsilon^2 \vert M_2 \vert} =  \dfrac{2 \cdot \vert E(F) \vert \cdot \vert M_2 \vert}{t^2}. $$
%\item $\vert M_2 \vert < \dfrac{\sqrt{n}}{\varepsilon^2}$: As in the last section, let $u=\underset{v\in F}{\text{argmax }}\text{deg}(v)$.
%\begin{enumerate}
%\item $\text{deg}(u) \geq \dfrac{2\cdot \sqrt{n}}{(1-\frac{1}{\sqrt{n}}) \cdot \varepsilon^3}$: We know that $estimate_1$ is bounded from below by $\frac{1-\frac{1}{\sqrt{n}}}{2}\cdot\text{deg}(u) \geq \sqrt{n} / \varepsilon^3 > \vert M_2 \vert / \varepsilon$. Therefore, it is enough to set $t = \sqrt{n}/\varepsilon^2$. Then we have
%$$ s \geq 2 \cdot \dfrac{\vert E(F) \vert}{\sqrt{n}} = 2 \cdot \dfrac{\vert E(F) \vert \cdot \sqrt{n}}{ \varepsilon^4 t^2} >  \dfrac{2 \cdot \vert E(F) \vert \cdot \vert M_2 \vert}{t^2}. $$
%Note that this also means that it is sufficient to simply output $estimate_1 + \sqrt{n}/\varepsilon^2$ since $$\vert M_1 \vert + \vert M_2 \vert < estimate_1 + \sqrt{n}/\varepsilon^2 \leq \vert M_1 \vert + \varepsilon \cdot estimate_1 \leq (1+\varepsilon)(\vert M_1 \vert + \vert M_2 \vert). $$
%\item $\text{deg}(u) < \dfrac{2\cdot \sqrt{n}}{(1-\frac{1}{\sqrt{n}}) \cdot \varepsilon^3}$: If $estimate_1 \geq \dfrac{\sqrt{n}}{\varepsilon^3}$ then we can do the same analysis as in case $a)$. If $estimate_1 < \dfrac{\sqrt{n}}{\varepsilon^3}$ then we can bound the number of edges in the whole graph by 
%$$ \vert E \vert \leq \vert E(F) \vert + n \cdot estimate_1 = O(n^{1.5}/\varepsilon^3) $$
%where the last estimation follows from the fact that 
%$$ \vert E(F) \vert \leq \vert F \vert \cdot \frac{1}{\sqrt{n}}\text{deg}(u)\leq \sqrt{n}\cdot\text{deg} (u) = O(\dfrac{n}{\varepsilon^3}). $$ 
%Thus, due to the coupon collector's problem our sample $S$ contains every edge from $E$ (and $E(F)$) with high probability.
%\end{enumerate}
%\end{enumerate}
%
%According to Lemma \ref{lem:trivialest}, we need $s \geq \dfrac{2 \cdot \vert E(F) \vert \cdot \vert M_2 \vert}{t^2}$ samples to have $\left\vert estimate_2 - \vert M_2 \vert \right\vert \leq t$ with constant probability. Therefore, our estimator $estimate_1 + estimate_2$ is either a $(1 \pm \varepsilon)$-approximation on the size of the maximal matching $M_1 \cup M_2$ (case 1, 2.a and first part of 2.b ) or is equal to $\vert M_1 \cup M_2 \vert$ (last part of case 2.b).
%
%For the rescaling of the estimate obtained in the second phase by $\frac{|E(F)|}{s}$, we additionally require an estimation of $E(F)$. We do this in a similar way as we estimate the maximal matching size in $|E(F)|$. We sample $n^{3/2}$ edges uniformly at random from $E$ and count the number of edges from $E(F)$ and scale this number by $\vert E \vert / n^{3/2}$. If $\vert E(F) \vert \geq \sqrt{n} / \varepsilon^2$ this gives us an $(1 \pm \varepsilon)$-approximation on the size of $E(F)$ (using Chebyshev). If $\vert E(F) \vert < \sqrt{n} / \varepsilon^2$ we also know that $\vert M_2 \vert < \sqrt{n} / \varepsilon^2$, \ie we are in case $2$ of the above case study. Recalling this case, it is either not necessary to estimate $\vert M_2 \vert$ at all (case 2.a, first part of 2.b) or we sample all edges from $E(F)$ (last part of case 2.b). Since we sample at least $n^{3/2} \cdot \frac{\vert E(F) \vert}{\vert E \vert}$ from $E(F)$ with high probability and we can easily check whether we have sampled the whole graph, we are able to distinguish between these cases.
%Additionally folding in the approximation of $|E(F)|$ results in a $\left(\frac{1}{2}-\epsilon,1+3\epsilon\right)$ approximation after rescaling with the approximation of $|E(F)|$.
%
%
%%For this, we need the following definition.
%
%%Here we apply $\ell_0$ sketches not for the adjacency matrix but for matrices defined as follows.
%%\begin{definition} Given an unweighted graph $G = (V,E)$, let the $n\times {n\choose 2}$ matrix $A_G$ with entry $(i,(j,k))\in [n]\times {[n]\choose 2}$ be defined by
%%\[a_{i,(j,k)} = \begin{cases} 1 & \text{if } i=j \text{ and } (v_j,v_k)\in E \\
%%0 & \text{if } i=k \text{ and } (v_j,v_k)\in E \\
%%0 & \text{otherwise}
%%\end{cases}\]
%%and let the $n\times {n\choose 2}$ matrix $A_G'$ with entry $(i,(j,k))\in [n]\times {[n]\choose 2}$ be defined by
%%\[a_{i,(j,k)}' = \begin{cases} 0 & \text{if } i=j \text{ and } (v_j,v_k)\in E \\
%%1 & \text{if } i=k \text{ and } (v_j,v_k)\in E \\
%%0 & \text{otherwise.}
%%\end{cases}\]
%%\end{definition} \noindent
%%We maintain an $\ell_2$ for each row $a_i$ of $A_G$ and $a_i'$ $A_G'$. 
%%%sampler of $\hat{a_i}$ and $\hat{a_i}'$. 
%%Let $a = \sum_{v\in F} a_v$ and $a' = \sum_{v\in F} a_v'$. Then the following holds 
%%\begin{enumerate}
%%\item $a_{(j,k)} = a'_{(j,k)} = 1$ for every edge $(v_j,v_k) \in E(F)$,
%%\item $a_{(j,k)} = 1 = 1-a'_{(j,k)}$ for $v_j \in F$, $v_k \not\in F$ and $(v_j,v_k) \in E$,
%%\item and $a_{(j,k)} = 0 = 1-a'_{(j,k)}$ for $v_j \not\in F$, $v_k \in F$ and $(v_j,v_k) \in E$.
%%\end{enumerate} 
%%\noindent Then we have $\langle a, a' \rangle = 2 \cdot \vert E(F) \vert$ which we can approximate using the $\ell_2$-sketches (TODO).
%%Then $\hat{a}$ is an $\ell_0$ sampler of $E\cap (F\times F)$.
%%Thus for each randomly chosen edge of the second phase we require $2 n $ $\ell_0$ samplers of size $O(\log^3 n)$ for a total space requirement in $O(n^{2-\epsilon}\cdot \epsilon^{-2}\cdot \log^3 n$. 
%
%All random coins used by the algorithm can be drawn from a seed of length $O(g(n)\cdot \log n)$, where $g(n)$ is the space requirement of the algorithm using pseudorandom generators for bounded space computation, see Nisan~\cite{Nis92} for more details. The total space requirement for the entire algorithm is therefore in $\tilde{O}(n^{3/2}\cdot \epsilon^{-2})$.
%\end{proof}
%
%\section{Much Simpler Proof: Unweighted Matching}
%
%\begin{algorithm}[h]
%\label{alg1.1}
%\caption{\bf{Unweighted Matching Approximation}}
%$M' \leftarrow \emptyset$\;
%$count \leftarrow 0$\;
%\For{$j=1 ${\bf{ to }$s$}}{
%Sample a random edge $e = (u,v)$ from $E(F)$\;
%\If{$u$ and $v$ are free w.r.t. $M'$ or $e \in M'$}{
%$count \leftarrow count + 1$\;
%$M' \leftarrow M' \cup e$\;
%}
%}
%\Return $count \cdot \frac{|E(F)|}{s}$\;
%\end{algorithm}
%\begin{lemma}
%\label{lem:trivialest2}
%Let $G(V,E)$ be an unweighted undirected graph and let $M_{OPT}$ be a maximum matching of $G$. Let $e_1,\ldots,e_s$ be a sequence of $s$ uniformly sampled edges of $E$. For each $1 \leq i \leq s$ denote by $X_i$ the binary random variable indicating if algorithm \ref{alg1.1} increased the counter by $1$ in the $i$-th iteration of the loop, that is 
%$X_i = 1$ iff $e_i \in M'$. Then we have
%$$ \frac{(1-\varepsilon)}{2} \cdot \vert M_{OPT} \vert \leq \sum_{i=1}^s X_i\cdot \frac{|E|}{s} \leq (1+\varepsilon) \cdot \vert M_{OPT} \vert$$
%with probability at least $\frac{1}{2}$ if $s \geq \frac{2 \vert V \vert}{\varepsilon^2}$.
%
%\[\mathbb{P}\left[ \left| \sum_{i=1}^s X_i\cdot \frac{|E|}{s}-|M| \right| < t\right] > \frac{1}{2}\]
%if $s\geq \frac{2 \cdot |E|\cdot |M|}{t^2}$.
%\end{lemma}
%\begin{proof}
%The probability of $X_i = 1$ is at least the size of the smallest maximal matching divided by $\vert E \vert$. Since $M'$ is a matching it is
%$$ \dfrac{\vert M_{OPT} \vert}{2 \cdot \vert E \vert} \leq \mathbb{P}\left[ X_i = 1 \right] \leq \dfrac{\vert M_{OPT}}{\vert E \vert}$$
%$$\text{Var}\left[ X_e \right] = \dfrac{\vert M \vert}{\vert E \vert} - \dfrac{\vert M \vert^2}{\vert E \vert^2} \leq \dfrac{\vert M \vert}{\vert E \vert}. $$
%We then have
%\begin{eqnarray}
%\label{eq:chebyshev}
%\mathbb{P}\left[ \left| |M'|\cdot \frac{|E|}{s}-|M| \right| \geq t\right] &\leq & \frac{\text{Var}\left[\sum_{e\in E'} X_e\cdot \frac{|E|}{s}\right]}{t^2}\\
%\label{eq:independence}
%& = &  \frac{\frac{|E|^2}{s^2} \sum_{e\in E'} \text{Var}\left[ X_e \right]}{t^2}\\
%\nonumber
%& \leq & \frac{|E|\cdot |M|}{s \cdot t^2}
%%\nonumber
%%&=&  \frac{|E|\cdot |M| }{s\cdot t^2},
%\end{eqnarray}
%where (\ref{eq:chebyshev}) follows from Chebyshev and (\ref{eq:independence}) follows from the independence of the $X_e$ variables.
%\end{proof}
\section{Unweighted Matching}
\label{sec:unweighted}
\vspace{-0.2cm}
\subsubsection*{Estimating the Matching Size of Trees in Dynamic Streams:}
\label{sec:unweighted_tree}

Let $T = (V,E)$ be a tree with at least $3$ nodes and let $h_T$ be the number of internal nodes, \ie nodes with degree greater than $1$. It is easy to see that the matching size is bounded by $h_T$ since every edge in a matching has to be incident to at least $1$ internal node. A maximum matching is also lower bounded by $h_T/2$ which is a consequence of Hall's Theorem. Therefore, it suffices to estimate the number of internal nodes of a tree to approximate the maximum matching within $2+\varepsilon$ factor which was also observed in \cite{EHL15}. In order to estimate the matching size, we maintain a $\ell_0$-Estimator for the degree vector $d \in \mathbb{R}^n$ such that $d_i = deg(v_i)-1$ holds at the end of the stream and with it $\ell_0(d) = h_T$. In other words, we initialize the vector by adding $-1$ to each entry and update the two corresponding entries when we get an edge deletion or insertion. Using Theorem 10 from~\cite{KNW10} we can maintain the $\ell_0$-Estimator for $d$ in $O(\varepsilon^{-2}\log^2 n)$ space. As in \cite{EHL15} this algorithm can be extended to forests with no isolated node.
\vspace{-0.1cm}
\begin{theorem}
Let $T = (V,E)$ be a tree with at least $3$ nodes and let $\varepsilon \in (0,1)$. Then there is an algorithm that estimates the size of a maximum matching in $T$ within a $(2+\varepsilon)$-factor in the dynamic streaming model using $1$-pass over the data and $O(\varepsilon^{-2}\log n)$ space.
\end{theorem}

%As in \cite{EHL15} this algorithm can be extended to forests with no isolated node.
\vspace{-0.7cm}
\subsubsection*{Dynamic Streaming Algorithms for Estimating the Matching Size in Graphs with Bounded Arboricity:}
\label{sec:unweighted_arboricity}

Let $G = (V,E)$ be a graph. The arboricity $a(G)$ of $G$ is a kind of density measure: The number of edges in every induced subgraph of size $s$  in $G$ is bounded by $s \cdot a(G)$. Formally, the arboricity $a(G)$ of $G$ is defined by $a(G) = \max\limits_{U \subseteq V} \left\lceil \frac{\vert E(U) \vert}{\vert U \vert -1} \right\rceil$.
If $\mu_G$ is an upper bound on the average degree of every induced subgraph of $G$ then $\mu_G \leq 2 \cdot a(G)$. Matchings in graphs with bounded arboricity were first studied by Czygrinow et al. \cite{CzygrinowHS09} for distributed computation of a $(1+\varepsilon)$-approximation. They divide the graph into nodes with low and high degree w.r.t. the arboricity such that it roughly suffices to approximate the matching in the bounded degree graph. 
Similarly, the estimation algorithms by Esfandiari et al. \cite{EHL15} 
%used the same idea to 
approximate the number of high degree nodes and the number of edges between the low degree nodes.
\vspace{-0.15cm}
\begin{definition}[\cite{EHL15}]
A node $v \in V$ is \emph{light} if $deg(v) \leq C$ with $C = \lceil \mu_G \rceil + 3$. Otherwise, $v$ is \emph{heavy}. An edge is \emph{shallow} if and only if both of its endpoints are light. We denote by $h_G$ the number of heavy nodes in $G$ and by $s_G$ the number of shallow edges in $G$, respectively.
\end{definition}
\vspace{-0.15cm}
Using the results from \cite{CzygrinowHS09} (and $C = 20a/\varepsilon^2$) it is possible to get a $O(a(G))$ approximation for the size of a maximum matching by just estimating $h_G$ and $s_G$. Esfandiari et al. \cite{EHL15} improve the approximation factor to roughly $5 \cdot a(g)$.
\vspace{-0.1cm}
\begin{lemma}[\cite{EHL15}]
\label{lem:match_arboricity}
Let $G = (V,E)$ be a graph with maximum matching size $M^*$. Then we have 
$ \frac{\max{\lbrace h_G, s_G \rbrace}}{\eta} \leq M^* \leq h_G + s_G$
where $\eta = 1.25 C + 0.75$. For graphs with bounded arboricity, the constant $C$ is at most $\lceil 2 a(G) +3 \rceil$.
\end{lemma}
\vspace{-0.1cm}
For heavy nodes, randomly drawing a large enough set of nodes, counting the heavy nodes by maintaining their degree and rescaling gives a sufficiently good estimate, provide $h_G$ is large enough. For shallow edges we only describe the single pass algorithm.
%the authors give two algorithms, one with smaller space requirement but requiring two passes and one with slightly larger space requirement $\tilde{O}(n^{2/3})$ implementable in a single pass. 
%The first one draws a random number of edges in the first pass and counts the number of shallow edges in the second, finally rescaling the estimate. 
The algorithm randomly draws nodes and maintains the induced subgraph. For each node contained in the subgraph it is straightforward to maintain the degree and thereby 
%to decide whether or not the node is heavy and 
to decide whether or not a given edge from the subgraph is shallow. The space requirement of approximating any value greater or equal some threshold $T$ is roughly $\tilde{O}(n/T)$ for heavy nodes and two-pass shallow edges and $\tilde{O}(n/\sqrt{T})$ for single pass shallow edges, making these estimation routines only feasible for large matching sizes. Therefore, the authors greedily maintain a maximum matching up to size $T$ and switch to estimating $h_G$ and $s_G$ if the size of the maximum matching exceeds a given threshold. Adapting the estimation algorithms for $h_G$ and $s_G$ for dynamic streams is straightforward. However, the greedy algorithm cannot be simulated in dynamic streams, even when allowing two passes over the data. Instead, we use the aforementioned rank decision problem on the Tutte-matrix of the graph for small matching values at the cost of space increase.
% 
%For a single pass, we approximate the rank of the Tutte-matrix of the graph. The entries of the Tutte-matrix $A$ are defined \[A_{ij} = \begin{cases} x_{ij} & \text{if }(i,j)\in E \text{ and }i<j \\
%-x_{ij} & \text{if }(i,j)\in E \text{ and }i>j\\
%0 &\text{otherwise}\end{cases},\]
%where $x_{i,j}$ are indeterminantes. Tutte~\cite{Tut47} showed that if there exists an assignment of the $x$, such that the determinant of $A$ is non-zero and hence $A$ has full rank, the graph has a perfect matching. This was generalized by Lov{\'{a}}sz~\cite{Lov79} who showed that the rank of $A$ is twice the size of the maximum matching. Furthermore, Lov{\'{a}}sz also noted that $A$ has maximum rank with high probability if the indeterminantes are chosen independently and uniformly at random from $\{1,\ldots, \text{poly}(n)\}$.
%
%Deciding whether a $n\times n$ matrix streamed via turnstile updates has rank at least $k$ is possible using $O(k^2\log n)$ space, see for instance Clarkson and Woodruff~\cite{CW09} and Andoni and Nguyen~\cite{AnN13}.

%Before proving our main theorem, we restate three technical lemmas from~\cite{EHL15} for arbitrary parameters.
%
%\begin{lemma}[\cite{EHL15}]
%\label{lem:heavy}
%Let $T$ be an integer. Then there exists a $1$-pass algorithm for $(1\pm \varepsilon)$ estimating any value of $h_G\geq T$ or outputting at most $4T$ if $h_G < T$ using $O(\frac{\log^2 n}{\varepsilon^2} \frac{n}{T})$ space.
%\end{lemma}
%\begin{proof}
%The probablity of sampling a heavy node is $\frac{h_G}{n}$. Hence, sampling a set of nodes $S$ gives us $|S|\cdot \frac{h_G}{n}$ heavy nodes on expectation. Set $|S|=\frac{3\log n}{\epsilon^2} \frac{n}{T}$. For each node $v\in S$ we maintain its degree using $O(\log n)$ space. We define the indicator variable $X_v$ which is $1$ if $v$ is heavy and $0$ otherwise. Then our estimator for $h_G$ is $\hat{h} = \frac{n}{\vert S \vert} \sum X_v$ which is equal to $h_G$ in expectation. First, assume $h\geq T$. Then using the Chernoff bound, we have
%\begin{eqnarray*}
%\mathbb{P}\left[ \left\vert \hat{h} -  \mathbb{E}\left[ \hat{h} \right]\right\vert > \varepsilon \cdot\mathbb{E}\left[\hat{h} \right]\right] & = & \mathbb{P}\left[ \left\vert \sum_{v\in S} X_v -  \mathbb{E}\left[ \sum_{v\in S} X_v\right]\right\vert > \varepsilon \cdot\mathbb{E}\left[ \sum_{v\in S} X_v\right]\right]\\
%&\leq & \exp\left( - \frac{3\log n}{\epsilon^2} \frac{n}{T} \cdot \frac{h_G}{n}\cdot \frac{\epsilon^2}{3} \right) \leq \frac{1}{n}.
%\end{eqnarray*}
%
%If $h_G < T$, then again using the Chernoff bound
%\begin{eqnarray*}
%\mathbb{P}\left[\frac{n}{|S|}\cdot\left(\sum_{v\in S} X_v\right) > 4T\right] &=& \mathbb{P}\left[\sum_{v\in S} X_v - \mathbb{E}\left[\sum_{v\in S} X_v\right] > \frac{4 T\cdot |S|\cdot h_G}{n\cdot h_G}-\mathbb{E}\left[\sum_{v\in S} X_v\right]\right]\\
%&=& \mathbb{P}\left[\sum_{v\in S} X_v - \mathbb{E}\left[\sum_{v\in S} X_v\right] > \left(\frac{4T}{ h_G}-1\right)\cdot \mathbb{E}\left[\sum_{v\in S} X_v\right]\right]\\
%&\leq & \exp\left(-\frac{3\log n}{\epsilon^2} \frac{n}{T} \cdot \frac{h_G}{n}\cdot \frac{\frac{4T}{h_G}-1}{3}\right) \leq \frac{1}{n},
%\end{eqnarray*}
%where the last inequality follows if $\epsilon \leq \frac{1}{2}$.
%\end{proof}

%\begin{lemma}[\cite{EHL15}]
%\label{lem:shallow2}
%Let $T$ be an integer. Then there exists a $2$-pass algorithm for $(1\pm \varepsilon)$ estimating any value of $s_G\geq T$ or outputting at most $4T$ if $s_G < T$ using $O(\frac{a(G) \cdot n \log^2 n}{\varepsilon^2 T})$ space.
%\end{lemma}
%\begin{proof}
%In the first pass, we sample $\frac{2\log n}{\epsilon^2} \frac{a(G) \cdot n}{T}$ edges. For each node of a sampled edge, we maintain its degree in the second pass to decide whether a given edge is shallow or not. Hereafter, we reapply the analysis of Lemma~\ref{lem:heavy}.
%\end{proof}

%\begin{lemma}[\cite{EHL15}]
%\label{lem:shallow1}
%Let $T>\log n$ be an integer. Then there exists a $1$-pass algorithm for $(1\pm \varepsilon)$ estimating any value of $s_G\geq T$ or outputting at most $4T$ if $s_G < T$ using $O(\frac{a(G) \cdot n \log^2 n}{\varepsilon \sqrt{T}})$ space.
%\end{lemma}
%\begin{proof}
%Let $S$ be a set of $\frac{4n}{\varepsilon\sqrt{T}}$ randomly chosen nodes. We maintain the entire subgraph induced by $S$ and the degree of each node in $S$. Note that the number of edges in this subgraph is at most $a(G) \cdot |S|$. Let $e_1, \ldots, e_{s_G}$ be the shallow edges. Define $X_i=1$ if $e_i \in E(S)$ and $0$ otherwise. $X_i$ is Bernouilli distributed where the probability of both nodes being included in the subgraph follows from the hypergeometric distribution with population $n$, $2$ successes in the population, sample size $|S|$ and $2$ successes in the sample:
%\[p= \frac{\binom{2}{2}\binom{n-2}{|S|-2}}{\binom{n}{|S|}} = \frac{|S|\cdot (|S|-1)}{n\cdot (n-1)} \geq \dfrac{\vert S \vert^2}{2 n^2} = \dfrac{8}{\varepsilon^2 T}.\]
%Hence $Var[X_i]= p\cdot (1-p)\leq p$. For the covariance between two variables $X_i$ and $X_j$ we have two cases: If $e_i$ and $e_j$ do not share a node, then $X_i$ and $X_j$ cannot be positively correlated. If $e_i$ and $e_j$ share a node, we have
%\begin{eqnarray*}
%Cov[X_iX_j] &=& \mathbb{E}[X_iX_j]-\mathbb{E}[X_i]\mathbb{E}[X_j] \leq \mathbb{P}[X_i=X_j=1]\\
%&=&\frac{\binom{3}{3}\binom{n-3}{|S|-3}}{\binom{n}{|S|}} = \frac{|S|\cdot (|S|-1)\cdot (|S|-2)}{n\cdot (n-1)\cdot (n-2)} < p^{3/2}.
%\end{eqnarray*}
%By definition each node incident to a shallow edge has at most $C$ neighbors and therefore, we have at most $2C$ edges that share a node with a given shallow edge. In total, we can bound the variance of $X = \sum_{e_i \in E(S)} X_i$
%\begin{eqnarray*}
%Var\left[ X \right] &=& \sum_{e_i \in E(S)} Var[X_i] + \sum_{e_i,e_j \in E(S)} Cov[X_i,X_j] \\
%&\leq & p \cdot s_G + \sum_{\substack{
%   e_i,e_j\in E(S) \\
%   e_i,e_j \text{ adjacent}
%  }} Cov[X_i,X_j] \leq p \cdot s_G  + 2C \cdot s_G \cdot p^{3/2} \leq 2p \cdot s_G
%\end{eqnarray*} 
%Using Chebyshev's inequality we have for $s_G\geq T$
%\begin{eqnarray*}
%\mathbb{P}\left[\left\vert\frac{1}{p} \cdot X - \frac{1}{p}\mathbb{E}\left[ X \right]\right\vert > \epsilon\cdot \frac{1}{p}\mathbb{E}\left[ X \right]\right]& = & \mathbb{P}\left[\left\vert X - \mathbb{E}\left[ X \right]\right\vert > \epsilon\cdot \mathbb{E}\left[ X \right]\right]\\
%&\leq & \frac{Var\left[ X \right]}{\epsilon^2\mathbb{E}\left[ X \right]^2} \leq \frac{2p \cdot s_G}{\epsilon^2 p^2 \cdot s_G^2} \leq \frac{2}{\epsilon^2 T p} \leq \frac{1}{4}.
%\end{eqnarray*}
%
%If $s_G < T$, we have
%\begin{eqnarray*}
%\mathbb{P}\left[\frac{1}{p} \cdot X > 4T\right] &=& \mathbb{P}\left[ X - \mathbb{E}\left[ X \right] > 4 T p - \mathbb{E}\left[ X \right] \right]\\
%& \leq & \mathbb{P}\left[ X - \mathbb{E}\left[ X \right] > 3 T p \right] \\
%&\leq & \frac{ Var\left[ X \right]}{9 T^2 p^2} \leq \frac{2 p \cdot s_G}{9 T^2 p^2} \leq \frac{2}{9 T p} \leq \dfrac{\varepsilon^2}{36}.
%\end{eqnarray*}
%
%The estimator is then amplified in the standard way by outputting the median of $O(\log n)$ independent copies.
%\end{proof}

%Using random sampling, our main algorithmic tool, to estimate $h_G$ and $s_G$ is infeasible if these values are small. Therefore, we additionally maintain a small maximal matching of size at most $n^\alpha$ with $\alpha < 1$. If the maintained matching exceeds this value then we know that either $s_G$ or $h_G$ is greater than $n^\alpha/2$ by Lemma \ref{lem:match_arboricity} and our estimation of these parameters will be sufficiently accurate.

%In the insertion-only setting \cite{EHL15} the space bottleneck is the estimation of the shallow edges, which needs $\tilde{O}(n^{2/3})$ space for only one pass (which also requires that $\alpha = 2/3$). By allowing a second pass over the data, they showed that only $\tilde{O}(\sqrt{n})$ space is sufficient to estimate $s_G$ (and $\alpha = 1/2$). 
%Adapting the estimation algorithms \ref{alg_estimate_hg} and \ref{alg_estimate_sg} for $h_G$ and $s_G$ for dynamic streams is straightforward. However, maintaining a matching of size at most $n^\alpha$ in one pass is hard when edge deletions are allowed. Nevertheless, we show that a small matching can be maintained in two passes with sublinear (w.r.t. the number of edges) space by utilizing sparse recovery sketches. 

%Our algorithm is similar to the multipass algorithm by Latanzi et al. \cite{LaMSV11} which repeatedly samples $O(n^{1+1/p})$ (free) edges and finds a maximal matching in the sampled subgraph. They showed that after $p$ passes the matching is maximal with high probability. The number of edges in \cite{LaMSV11} has to be $n^{1+c}$ for some $c > 0$. Here, we only have a linear number of edges and we can not apply the same technique to maintain a small matching with sublinear space

%Replacing the subroutines in the estimation algorithm in \cite{fehlt} by Lemma \ref{lem:maintain_matching} and the adaptions of algorithm \ref{alg_estimate_hg} and \ref{alg_estimate_sg} for dynamic streams gives us the following result.
\vspace{-0.15cm}
\begin{theorem}
Let $G$ be a graph with $a(G) \leq \nu$. Let $\varepsilon \in (0,1/2)$ be an arbitrary positive values less than one. Then there exists an algorithm estimating the size of the maximum matching in $G$ within a $((5 \nu +9)(1+\varepsilon)^2)$-factor in the dynamic streaming model using a single pass over the data and $\tilde{O}(\nu \cdot n^{4/5})$ space or two passes over the data and $\tilde{O}(\nu \cdot n^{2/3})$ space.
\end{theorem}
%\begin{proof}
%%The first part of the theorem follows from Corollary~\ref{cor:2pass} and Lemmas~\ref{lem:heavy} and~\ref{lem:shallow2} with $T=\sqrt{n}$.
%For the first part of the theorem we assume that in Algorithm \ref{alg:unweighted_matching} each indeterminant of the Tutte-matrix independently gets a weight uniformly chosen from $\{1, \ldots, \text{poly}(n)\}$. Upon insertion or deletion of an edge we update the corresponding entry by the appropriate value. For all powers of $2$ less or equal than $18T$, we solve the rank decision problem on the Tutte-matrix of the graph where the indeterminantes have been replaced by the random values using a total of $O(T^2\log^2 n\log T ) = O(T^2\log^3 n)$ space. In addition, we estimate $s_G$ and $h_G$ by $\hat{h}$ and $\hat{s}$ using $\tilde{O}(\frac{\nu n}{\sqrt{T}})$ space, see Lemma~\ref{lem:shallow1} and Lemma \ref{lem:heavy}. Setting $T=n^{2/5}$ gives us the desired space bound. 
%If $\max\lbrace \hat{h}, \hat{s} \rbrace > 4T$ we know that $\max\lbrace \hat{h}, \hat{s} \rbrace$ approximates the value of $\max\lbrace h_G, s_G \rbrace$ and output $\dfrac{\max\lbrace \hat{h}, \hat{s} \rbrace}{(1+\varepsilon) \eta}$ as an estimation for the matching size. Using Lemma \ref{lem:match_arboricity} it holds
%$$ \dfrac{\max\lbrace \hat{h}, \hat{s} \rbrace}{(1+\varepsilon) \eta} \leq M^* \leq h_G+s_G \leq 2(1+\varepsilon)\max\lbrace \hat{h}, \hat{s} \rbrace. $$
%If $\max\lbrace \hat{h}, \hat{s} \rbrace < 4T$ we know that $M^* \leq 9 T$. Thus, we can use the rank decisions to estimate the size up to a factor of $2$.
%Besides the random bits for the Tutte-matrix the algorithm uses $\tilde{O}(\nu \cdot n^{4/5})$ for the single pass estimation of $s_G$. Using Nisan's pseudo random generators for bounded space computation~\cite{Nis92} the random bits can be drawn from a seed of length $O(S \log n)$ (where $S$ is the space requirement of our algorithm).
%
%For the second part of the theorem we can improve the space requirements for the estimator $\hat{h}$ and $\hat{s}$ to $\tilde{O}(\frac{\nu n}{T})$ by using Lemma \ref{lem:heavy} and Lemma \ref{lem:shallow2}. Now, setting $T = n^{1/3}$ gives the desired result.
%\end{proof}



%\begin{algorithm}[h]
%\label{alg_estimate_hg}
%\caption{\bf{Heavy nodes}}
%%\LinesNumbered
%\SetKwData{I}{i}
%\SetKwInOut{Input}{input}
%\Input{A stream of edge insertions and deletions}
%Initialize $V' \subset V$ as a random subset of size $3 \cdot \varepsilon^{-2} \sqrt{n}$.\\
%For every $v \in V'$, initialize $deg(v)$ to zero.\\
%\textbf{Insertion of $e = (u,v)$:}\\
%\If{$u \in V'$}{
%$deg(u) = deg(u)+1$
%}
%\If{$v \in V'$}{
%$deg(v) = deg(v)+1$
%}
%\textbf{Deletion of $e = (u,v)$:}\\
%\If{$u \in V'$}{
%$deg(u) = deg(u)-1$
%}
%\If{$v \in V'$}{
%$deg(v) = deg(v)-1$
%}
%\textbf{End of stream:}\\
%Let $h' = \vert \lbrace v \in V' \mid deg(v) > \mu \rbrace \vert$ denote the number of heavy nodes in $V'$.\\
%Return $\hat{h} = h' \cdot \dfrac{\sqrt{n}}{3 \cdot \varepsilon^{-2}}$.
%\end{algorithm}
%
%\begin{algorithm}[h]
%\label{alg_estimate_sg}
%\caption{\bf{Shallow Edges using 2 Passes}}
%%\LinesNumbered
%\SetKwData{I}{i}
%\SetKwInOut{Input}{input}
%\Input{A stream of edge insertions and deletions}
%\textbf{First Pass:}\\
%Let $S$ be a random sample set of edges chosen with probability $\dfrac{2 \log(4/\delta)}{\varepsilon^2 \sqrt{n}}$\;
%\textbf{Second Pass:}\\
%$E' := \emptyset$\;
%\For{each edge $e \in S$}{
%\If{$e$ is shallow}{
%Add $e$ to set $E'$\;
%}
%}
%Return $\hat{s} = \vert E' \vert \cdot \dfrac{\varepsilon^2 \sqrt{n}}{3 \log(4/\delta)}$.
%\end{algorithm}

%\begin{algorithm}[h]
%\caption{\bf{Unweighted Matching Approximation}}
%%\LinesNumbered
%\SetKwData{I}{i}
%\SetKwInOut{Input}{input}
%\Input{$G=(V,E)$ with $a(G) \leq \nu$, $1/2 > \varepsilon > 0$}
%Set $T = n^{2/5}$ and $\eta = 2.5\nu+5.75$.\\
%Let $\hat{h}$ and $\hat{s}$ be the estimators from Lemma \ref{lem:heavy} and Lemma \ref{lem:shallow1}.\\
%\For{$i=1, \ldots, \lceil \log 18T \rceil$}{
%Solve rank decision with parameter $k = 2^i$ on the Tutte-Matrix $T$ with randomly chosen indeterminants.
%}
%\eIf{$\max\lbrace \hat{h}, \hat{s} \rbrace > 4T$}{
%Output $\dfrac{\max\lbrace \hat{h}, \hat{s} \rbrace}{(1+\varepsilon) \eta}$.}{
%Output $\max k \in \lbrace 1,\ldots , 2^{\lceil \log 18T \rceil} |~||T||_{S0}\geq k \rbrace $.
%}
%\end{algorithm}

%
%Esfandiari et al. \cite{fehlt} also showed that it is possible to estimate the size of a maximum matching in a forest by estimating the number of nodes with degree $2$ or more. 
%\begin{lemma}[\cite{fehlt}]
%Let $F$ be a forest with $c_F$ connected components and no isolated node. Let $OPT$ be the size of a maximum matching and let $h_F$ denote the number of nodes with degree $2$ or more. Then we have
%$$ \dfrac{h_F+c_F}{2} \leq OPT \leq h_F + c_F. $$
%\end{lemma}


%\section{Estimation in General Graphs}
%Let the set of edges $E$ of graph be a matching. We seek to estimate $m=|E|$ by randomly sampling a set $S$ of $k$ nodes and storing the induced subgraph, that is $E(S)=(S\times S)\setminus E$. Let $X_S$ denote the event that $E(S)\neq \emptyset$. On expectation, a $2m/n$ fraction of nodes in $S$ will be matched nodes.
%
%Our aim is to find bounds on $k$, depending on $n$ and $m$ such that the complementary event $X_S$ has probablity greater than $\frac{1}{2}$.
%
%Taking the logarithm gives
%\begin{eqnarray}
%\sum_{i=0}^m \log \mathbb{P}[X_S=0] &=& \sum_{i=0}^{m-1} \log \left(1-\frac{\binom{k}{2}}{\binom{n}{2}-i}\right) \leq \sum_{i=0}^{m-1} - \frac{\binom{k}{2}}{\binom{n}{2}-i} \leq - m\cdot \frac{\binom{k}{2}}{\binom{n}{2}}
%\end{eqnarray}
%and
%
%\begin{eqnarray}
%\sum_{i=0}^m \log \mathbb{P}[X_S=0] &=& \sum_{i=0}^{m-1} \log \left(1-\frac{\binom{k}{2}}{\binom{n}{2}-i}\right) \geq \sum_{i=0}^{m-1} - c\cdot \frac{\binom{k}{2}}{\binom{n}{2}-i} \geq - m\cdot \frac{c\cdot \binom{k}{2}}{\binom{n}{2}-m}
%\end{eqnarray}
%where $c$ is a sufficiently large constant. Since $m< n/2$, the upper and lower bounds differ by only a constant factor. Hence setting the probability of event $X_S$ to $\frac{1}{2}$ gives us the asymptotic bounds ${k\choose 2}\in \Theta \left(\frac{n^2}{m}\right) \Leftrightarrow k\in \Theta \left(\frac{n}{\sqrt{m}}\right)$.
%
%We can verify a given estimate $m$ via multiple independently chosen copies of $S$ and applying Chernoff bounds. Further using an exponentially increasing sequence of estimates for $m$ starting with a minimal estimate $m_0$, we can estimate any matching size greater than $m_0$ up to a constant factor using $O\left(\frac{n}{\sqrt{m_0}}\log n\right)$ space.
\vspace{-0.1cm} \noindent
We want to mention that it is also possible to maintain a small matching in $2$-passes using only sublinear space w.r.t. $\vert E \vert$ in a dynamic stream. This algorithm can also be used for the $2$-pass algorithm above also using $\tilde{O}(\nu n^{2/3})$ space.
\vspace{-0.1cm}
\begin{lemma}
\label{lem:maintain_matching}
Let $G$ be a graph with $m$ edges and let $\alpha_1 \in (0,1]$ and $\alpha_2 \in (0,2)$ with $\alpha_1 \leq \alpha_2$. There is a dynamic streaming algorithm that maintains a matching of size $n^{\alpha_1}$ in space $\tilde{O}(\frac{m}{n^{\alpha_2}} \cdot n^{\alpha_1} + n^{\alpha_2})$ using two passes with high probability.
\end{lemma}
%\begin{proof}
%We denote by $F$ the unmatched nodes w.r.t. some matching (which is clear from the content). Let $M$ be some matching and assume that $\vert E(F) \vert$ is large. If we repeatedly sample an edge uniformly at random, then we will see a edge from $E(F)$ after a small number of steps with high probability. If we continue this process long enough and update our matching $M$ every time we see an free edge, we have either found a large matching or the remaining number of free edges is small.
%
%Let $T = 2 \cdot \frac{m}{n^{\alpha_2}} \cdot n^{\alpha_1}$. In the first pass we sample a sequence $(e_1, \cdots, e_T)$ of $T$ edges uniformly at random. After each sampled edge we update a matching $M_1$ (starting with an empty matching) by adding an edge to $M_1$ iff both endpoints are currently unmatched. If after the first pass $M_1$ is smaller than $n^{\alpha_1}$, we build an $n^{\alpha_2}$-recovery sketch (see Definition \ref{def:recovery_sketch}) for the edges in $E(F)$ where $F$ is the set of unmatched nodes.
%
%Let $F_i$ be the set of unmatched nodes before we sample edge $e_i$, \ie $F_1 = V$, and let $F_{T+1}$ be the set of unmatched nodes after the first pass. Assume that $\vert E(F_{T+1}) \vert \geq n^{\alpha_2}$. Then we know that $\vert E(F_i) \vert \geq n^{\alpha_2}$ for every $1 \leq i \leq T$. Let $X_i = 1$ iff $e_i \in E(F_i)$ and let $X = \sum_{i=1}^T X_i$, \ie $\vert M_1 \vert = \min\lbrace n^{\alpha_1}, X \rbrace$. It is
%$$ E\left[ X \mid \vert E(F_{T+1}) \vert \geq n^{\alpha_2} \right] \geq T \cdot \dfrac{n^{\alpha_2}}{m} = 2 \cdot n^{\alpha_1}. $$
%Since adding an edge to $M_1$ at step $i$, \ie $X_i = 1$, decreases the probability that $X_j = 1$ for $j > i$ while $X_i = 0$ does not influence the probabilities, these random variables are negatively correlated. Thus, we can use Chernoff bounds to prove that
%$$ \mathbb{P}\left[ X < n^{\alpha_1} \mid \vert E(F_{T+1}) \vert \geq n^{\alpha_2} \right] \leq \mathbb{P}\left[ X < (1/2) E\left[ X \right] \mid \vert E(F_{T+1}) \vert \geq n^{\alpha_2} \right] \leq e^{-n^{\alpha_1}/4} $$
%which gives us
%\begin{eqnarray*}
%\mathbb{P}\left[ X < n^{\alpha_1} \wedge \vert E(F_{T+1}) \vert \geq n^{\alpha_2} \right] & = & \mathbb{P}\left[ X < n^{\alpha_1} \mid \vert E(F_{T+1}) \vert \geq n^{\alpha_2} \right] \cdot  \mathbb{P}\left[ \vert E(F_{T+1}) \vert \geq n^{\alpha_2} \right]\\
%& \leq & \mathbb{P}\left[X < n^{\alpha_1} \mid \vert E(F_{T+1}) \vert \geq n^{\alpha_2} \right] \leq  e^{-n^{\alpha_1}/4}.
%\end{eqnarray*}
%Therefore, we have either $\vert M_1 \vert = n^{\alpha_1}$ or $\vert E(F_{T+1}) \vert < n^{\alpha_2}$ after the first pass with high probability. 
%
%Sampling $T$ edges can be done by $T$ $\ell_0$-sampler in space $\tilde{O}(T)$. In the second pass we have the matching and an $n^{\alpha_2}$-recevory sketch where both can be maintain in $\tilde{O}(n^{\alpha_2})$ space.
%\end{proof}

%Graphs with arboricity $\nu$ can only have at most $\nu \cdot n$ edges.
\vspace{-0.1cm} \noindent By using Lemma $\ref{lem:maintain_matching}$ with $m = \nu \cdot n, \alpha_1 = 1/3$ and  $\alpha_2 = 2/3$ we can maintain a matching of size at most $n^{1/3}$ in space $\tilde{O}(\nu \cdot n^{2/3})$ in graphs with bounded arboricity $\nu$.
%\vspace{-0.1cm}
%\begin{corollary}
%\label{cor:2pass}
%There is a $2$-pass dynamic streaming algorithm using $\tilde{O}(\nu \cdot n^{2/3})$ space that maintains a matching of size at most $n^{1/3}$ in graphs with bounded arboricity $\nu$.
%\end{corollary}

